PISCOLA: a data-driven transient light-curve fitter

Forthcoming time-domain surveys, such as the Rubin Observatory Legacy Survey of Space and Time, will vastly increase samples of supernovae (SNe) and other optical transients, requiring new data-driven techniques to analyse their photometric light curves. Here, we present the "Python for Intelligent Supernova-COsmology Light-curve Analysis" (PISCOLA), an open source data-driven light-curve fitter using Gaussian Processes that can estimate rest-frame light curves of transients without the need for an underlying light-curve template. We test PISCOLA on large-scale simulations of type Ia SNe (SNe Ia) to validate its performance, and show it successfully retrieves rest-frame peak magnitudes for average survey cadences of up to 7 days. We also compare to the existing SN Ia light-curve fitter SALT2 on real data, and find only small (but significant) disagreements for different light-curve parameters. As a proof-of-concept of an application of PISCOLA, we decomposed and analysed the PISCOLA rest-frame light-curves of SNe Ia from the Pantheon SN Ia sample with Non-Negative Matrix Factorization. Our new parametrization provides a similar performance to existing light-curve fitters such as SALT2. We further derived a SN Ia colour law from PISCOLA fits over $\sim$3500 to 7000\AA, and find agreement with the SALT2 colour law and with reddening laws with total-to-selective extinction ratio $R_V \lesssim 3.1$.

==> tables/table_mb_comparison_multi_cadences.tex <==
\begin{table*}
\caption{Weighted mean ($\bar{x}_w$) and RMS of $\Delta$\mb. The sub-indices represent the cadence of the simulations (from 1 to 10 days).}
\tiny
\setlength\tabcolsep{1.5pt}
\begin{tabular}{lcccccccccc}
\hline
survey & $(\bar{x}_w \pm RMS)_1$            & $(\bar{x}_w \pm RMS)_2$           & $(\bar{x}_w \pm RMS)_3$           & $(\bar{x}_w \pm RMS)_4$           & $(\bar{x}_w \pm RMS)_5$           & $(\bar{x}_w \pm RMS)_6$           & $(\bar{x}_w \pm RMS)_7$           & $(\bar{x}_w \pm RMS)_8$           & $(\bar{x}_w \pm RMS)_9$           & $(\bar{x}_w \pm RMS)_{10}$          \\ 
 & [mag] & [mag] & [mag] & [mag] & [mag] & [mag] & [mag] & [mag] & [mag] & [mag] \\
\hline \hline
Low-z & 0.004 $\pm$ 0.013 & 0.003 $\pm$ 0.015 & 0.004 $\pm$ 0.021 & 0.004 $\pm$ 0.023 & 0.004 $\pm$ 0.026 & 0.005 $\pm$ 0.030 & 0.007 $\pm$ 0.037 & 0.010 $\pm$ 0.044 & 0.014 $\pm$ 0.063 & 0.025 $\pm$ 0.103  \\
SDSS & -0.020 $\pm$ 0.031 & -0.019 $\pm$ 0.036 & -0.020 $\pm$ 0.040 & -0.018 $\pm$ 0.037 & -0.018 $\pm$ 0.041 & -0.019 $\pm$ 0.042 & -0.027 $\pm$ 0.047 & -0.033 $\pm$ 0.058 & -0.036 $\pm$ 0.065 & -0.045 $\pm$ 0.083  \\
SNLS & -0.003 $\pm$ 0.012 & -0.002 $\pm$ 0.015 & -0.003 $\pm$ 0.018 & -0.002 $\pm$ 0.018 & -0.005 $\pm$ 0.021 & -0.002 $\pm$ 0.021 & -0.002 $\pm$ 0.021 & -0.006 $\pm$ 0.027 & -0.015 $\pm$ 0.038 & -0.025 $\pm$ 0.046  \\
PS1 & -0.009 $\pm$ 0.032 & -0.006 $\pm$ 0.036 & -0.007 $\pm$ 0.044 & -0.005 $\pm$ 0.045 & -0.005 $\pm$ 0.049 & -0.004 $\pm$ 0.051 & -0.009 $\pm$ 0.053 & -0.016 $\pm$ 0.055 & -0.022 $\pm$ 0.062 & -0.025 $\pm$ 0.062  \\ 
\hline
\end{tabular}
\label{tab:mb_com_multi_cad}
\end{table*}
